A Distributed Model-Free Ride-Sharing Approach for Joint Matching, Pricing, and Dispatching using Deep Reinforcement Learning

Significant development of ride-sharing services presents a plethora of opportunities to transform urban mobility by providing personalized and convenient transportation while ensuring efficiency of large-scale ride pooling. However, a core problem for such services is route planning for each driver to fulfill the dynamically arriving requests while satisfying given constraints. Current models are mostly limited to static routes with only two rides per vehicle (optimally) or three (with heuristics). In this paper, we present a dynamic, demand aware, and pricing-based vehicle-passenger matching and route planning framework that (1) dynamically generates optimal routes for each vehicle based on online demand, pricing associated with each ride, vehicle capacities and locations. This matching algorithm starts greedily and optimizes over time using an insertion operation, (2) involves drivers in the decision-making process by allowing them to propose a different price based on the expected reward for a particular ride as well as the destination locations for future rides, which is influenced by supply-and demand computed by the Deep Q-network, (3) allows customers to accept or reject rides based on their set of preferences with respect to pricing and delay windows, vehicle type and carpooling preferences, and (4) based on demand prediction, our approach re-balances idle vehicles by dispatching them to the areas of anticipated high demand using deep Reinforcement Learning (RL). Our framework is validated using the New York City Taxi public dataset; however, we consider different vehicle types and designed customer utility functions to validate the setup and study different settings. Experimental results show the effectiveness of our approach in real-time and large scale settings.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for IEEE conference papers.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl.tex          - A bare bones starter file for IEEE journal papers.

bare_jrnl_comsoc.tex   - A bare bones starter file for IEEE Communications
                         Society journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_jrnl_transmag.tex - A bare bones starter file for IEEE Transactions
                         on Magnetics journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for an IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_conf_compsoc.tex, bare_jrnl.tex,
                   bare_jrnl_comsoc.tex, bare_jrnl_compsoc.tex,
                   bare_jrnl_transmag.tex
***************************************************************************


==> intro_old.tex <==
\subsection{\textcolor{blue}{Motivation}}
Advanced user-centric ride-hailing services such as Uber and Lyft are thriving in urban environments by transforming urban mobility through convenience in travel to anywhere, by anyone, and at anytime. Given tens of millions of users per month \cite{2-2}, these mobility-on-demand (MoD) services introduce a new paradigm in urban mobility \textemdash ride-sharing or ride-splitting. These ride-hailing services, when adopting shared mobility, can provide an efficient and sustainable way of transportation \cite{36}. With higher usage per vehicle, its service can reduce traffic congestion, environmental pollution, as well as energy consumption, thereby enhance living conditions in urban environments \cite{40-37}.  \textcolor{blue}{The majority of earlier articles in literature consider static and deterministic Dial-A-Ride Problems (DARP)s.  The main focus of these articles is on algorithmic advancement where the typical setting considers a homogeneous fleet of vehicles,  passengers' pick-up and drop-off time windows,  maximum passenger ride time,  maximum route duration, and vehicle capacity.  (e.g.,  \cite{PARRAGH20101129, PARRAGH2013490, CHASSAING2016119, ritzinger2016dynamic}).  %Some papers include these requirements as hard constraints in their optimization models (e.g.,  \cite{CHASSAING2016119,ritzinger2016dynamic}), while others may allow violations that are then penalized in the objective function so as to be avoided as much as possible \cite{urra2015hyperheuristic}. 
 In \cite{zhan2016graph},  the taxi trip data in New York City is used to quantitatively examine the gap between the current system performance and the theoretically optimal system.  However, this study adopts a model-based approach to compute a theoretical bound and only considers taxi service that serve one ride at a time while not addressing issues that arise with pooling or shareability.  However, in \cite{santi2014quantifying},  authors introduce the notion of shareability network, which allows modelling the collective benefits of sharing as a function of passenger inconvenience,  and  they conclde the potential of a new taxi system in which trips are routinely shareable while keeping passenger discomfort low in terms of prolonged travel time.\\
As conclusded in \cite{HO2018395},  Dynamic and Stochastic DARPs appear to be the most challenging,  which is the focus of our paper, regarding the difficulties arising from the modeling of a combination of stochastic components,  and the evaluations of outcomes under a large number of scenarios.\\%the integration of stochastic processes and optimization algorithms,  and the timely provision of high-quality solutions for recovery.  \\
In addition,  the growth in demand coupled with the rise of self-driving technology points towards a need for a fleet management framework that accomodates both the drivers' and customers' preferences in an optimal and sustainable manner.  Even though the pooling services provide customized personal service to customers, both the drivers and the customers are largely left out in deciding what is best for them in terms of their conveniences and preferences. It is challenging to introduce customer and driver conveniences into the framework. For example, a customer may have limitation on the money to spend on a particular ride as well as time constraints on reaching the destination. On the other hand, driver may not be willing to accept the customer’s convenient fare as it may negatively affect his/her profits since the final destination may be in low demand area. Thus,  a reliable framework is needed to identify trade-offs between drivers’ and customers’ needs, and make a compromised decision that is favorable to both.  Our proposed intelligent transportation system, driven by the objective of maximizing utility and maintaining service levels that accomodates both drivers' and customers' preferences, has the potential to revolutionize transportation systems}.
\vspace{-.1in}
\subsection{\textcolor{blue}{Related Work}}
\textcolor{blue}{Some articles in literature aim to study the practical impacts of the modeling techniques of DARPs,  for instance, graph representation of the road network \cite{GARAIX201062}, and modeling issues regarding new features motivated by new applications of DARPs\cite{MOLENBRUCH201758}, \cite{schonberger2017scheduling}.  %discussed the problem of the graph representation of the road network where arcs are computed according to only a single criterion, for example, travel time; which could eliminate some possible routes from consideration.  Some works  \cite{MOLENBRUCH201758}, \cite{schonberger2017scheduling} focus on the modeling issues regarding new features motivated by new applications of DARPs or real needs in practice. 
However, the focus of this paper is to provide an effecient matching and distributed pricing and route-planning framework that accounts for both drivers' and customers' preferences, where the matching scheme is both demand-aware and pricing-based.}\\
\textcolor{blue}{
\textbf{Matching and Route-Planning:}}
An essential issue in realizing shared mobility in online ride-sharing settings is \textit{route planning}, which has been proven to be an NP-hard problem \cite{np,DARP,np2}. Route planning - given a set of vehicles $V$, and requests $R$ - designs a route that consists of a sequence of pickup and drop-off locations of requests assigned to each vehicle. In ride-sharing environments, vehicles and requests arrive dynamically and are arranged such that they meet different objectives (e.g., maximizing the fleet's profits \cite{10-DA,40-37} and the number of served requests \cite{14,44}, and minimizing the average delay among customers and the total travelling distance \cite{23,30,32}).\\
\textcolor{blue}{The assignment problem in urban transportation has been widely studied in literature,  \cite{agatz2012optimization} provides a review of optimization approaches in dynamic ride-sharing.  However, most of these approaches do not consider the preferences of both parties, they mostly optimize for the service provider profitability.  %In our approach, matches must be time-feasible,  where both the rider’s and the driver’s travel windows are respected. 
Many of the earlier algorithmic approaches that address the assignment problem in literature limit their attention to what is denoted as static ride-sharing variants, where it is assumed that all driver and rider requests are known in advance prior to the execution of a matching process as in \cite{herbawi2011evolutionary, CORTES2010711}.  In \cite{alonso2017demand},  authors propose a solution for the matching problem by identifying cliques of the vehicle-pasenger graph as the potential trips. Then, they formalize the assignment problem as an integer linear problem (ILP), similarly in \cite{tafreshian2020trip}. However,  these approaches are based on one-to-one matching and do not address dynamic route-planning where new ride requests can be served by a vehicle that might be already assigned a trip as long as it still has vacant seats. \\
In any practical dynamic ride-share implementation, new riders and drivers continuously enter and leave the system.  Therefore,not all relevant offers and requests may be known at the time the ride-share provider executes an algorithm for planning ride-sharing arrangements. In recent years, several authors have addressed this issue in dynamic ride-sharing.  In \cite{AGATZ20111450}, authors deal with this planning uncertainty by using a rolling horizon solution approach where the optimization problem includes all of the offered rides (drivers) and requested rides (riders) that are known at the time of execution and that have not yet been matched.  In a similar setting, but accounting for automated taxis,  \cite{liang2020automated} proposes an integer non-linear programming (INLP) model that optimizes the routing of the automated taxis to maximize the system profit. Similarly, \cite{kleiner2011mechanism} apply a rolling horizon solution approach as well where arrangements are committed as late as possible given the time considerations.  This is not always applicable in real-time and can lead to customer unsatisfaction on the long run.  Moreover, neither drivers' nor customers' preferences are taken into consideration in the decision-making process.  In \cite{zhang2020pricing}, authors address the allocation problem by modelling it as a bi-partitie matching, and address the drivers' scheduling problem by proposing a heuristic nearest neighbor algorithm that provides an approximate solution to the well-known hamiltonian path problem which is an NP-Hard problem. However, both are still one-to-one approaches that do not take into consideration which rides to group together. In attempt to further improve the matching problem,  \cite{liu2020mobility} proposes mT-share that fully exploits both real-time and historical mobility information of taxis and ride requests. In our DARM approach, we utilize near-future demand prediction to further optimize our matching.}\\
Utilizing an operation called \textit{insertion} to solve such a highly dynamic problem has been proven, in literature, to be both effective and efficient \cite{12,14,23,30,32,35,38,40-37,44}. The \textit{insertion} operation aims to accommodate the newly arriving request by inserting its pickup (i.e., origin) and its drop-off (i.e., destination) locations into a vehicle’s route. The main issue with the state-of-the-art route planning methods \cite{10-DA,12,40-37} is that it operates in a greedy fashion to optimize its objectives, which means each insertion operation only optimizes the objective function upon the \textit{current} arranged request leading to low performance over the long run. Moreover, most of the approximation algorithms that provide solutions to the route planning problem are limited to only two requests per vehicle such as the settings in \cite{np,np2,DARP}. In \cite{DARP}, the authors improve the effectiveness of route planning for shared mobility through taking into consideration the demand in near future (e.g., future 90 minutes), thus overcoming the short sightedness problem of the insertion operator. However, the Demand-Aware Route Planning (DARP) in \cite{DARP} is still limited to only two rides per vehicle in the initial assignment phase. \textcolor{blue}{In \cite{xu2020efficient}, authors study the time complexity of insertion operations, and propose a partition framework with dynamic programming that reduces the complexity from $O(n^{3})$ to $O(n^{2})$. For our DARM approach, we investigate the complexity of our approach in Section \ref{darm}. In \cite{li2020ride}, the authors extend the insertion algorithm proposed in \cite{campbell2004efficient} and consider travel-time uncertainty where they assume riders can change their ride information on-the-fly.  However,  their approach does not enforce constraints on which rides can be grouped together, which may result in grouping rides whose destinations are in opposite directions; thus resulting in large detours (boosting the travel distance), as well as extra fuel and energy consumption per vehicle.} Therefore, a robust framework is essential to achieve a dynamic and demand-aware matching framework that optimizes for the overall fleet's profits and travelling distance. Finally, the overall problem for ride-sharing requires interconnected decisions of matching, pricing, and dispatching, and is the focus of this paper. \\
In this paper, we present a dynamic, demand-aware and pricing-based vehicle-passenger matching and route-planning framework that scales up to accommodate more than two rides per vehicle (up to the maximum capacity of the vehicle) in the initial assignment phase followed by an optimization phase where the insertion operations are applied in order to achieve a matching that satisfies our platform-related set of constraints (as described in Section \ref{darm}). At the same time, we incorporate the pricing aspect to our matching algorithm which would prioritize the  rides with significant intersection in the path to be grouped together. This provides an efficient dynamic matching algorithm for the ride-sharing environment by managing the prices for the passengers based on the distance travelled after the insertion of the passenger in the route based on the previous passengers.

%Another problem  addressed in this paper is that even though the pooling services provide customized personal service to customers, both the drivers and the customers are largely left out in deciding what is best for them in terms of their conveniences and preferences. It is challenging to introduce customer and driver conveniences into the framework. For example, a customer may have limitation on the money she/he could spend for a particular ride as well as time constraints on reaching the destination. On the other hand, driver may not be willing to accept the customer’s convenient fare as it may negatively affect his/her profits since the final destination may be in low demand area. Thus, a reliable framework is needed to identify trade-offs between drivers’ and customers’ needs, and make a compromised decision that is favorable to both.
\textcolor{blue}{
\textbf{Pricing in Ridesharing:}
Regarding the pricing problem, there are various ways to divide the trip costs between the ride-share partners.  \cite{geisberger2009fast} suggests to divide the cost of the shared part of the trip evenly between the ride-share partners.  In \cite{AGATZ20111450},  authors propose a way to allocate the costs of the joint trip that is proportional to the distances of the separate trips.  \cite{kleiner2011mechanism} proposes an auction-based mechanism to determine the driver’s compensation. %This approach takes into account the different ride valuations of individual riders.  
Most works in literature study ride-sourcing pricing based on the steady-state equilibrium approach.  In \cite{cachon2017role}, authors study surge-pricing as a revenue management strategy. They consider a two-period newsvendor model to study the impact of contractual agreements for ‘self-scheduling’ agents. %i.e., drivers that choose their own work-shifts in ride-sourcing markets.  
However,  the requirements for a stationary equilibrium as well as the assumption of time-invariant fleet size are strict and rarely prevailing in reality. \\
The authors in \cite{nourinejad2019ride} consider a non-equilibrium two-sided markets, however they propose a model-based approach that introduces a three-state model (riders, vacant ride-sourcing vehicles, and occupied ride-sourcing vehicles) where the arrivals of vehicles and riders are endogenously dependent on the market state. Many researchers focus on the interactions and endogeneity between various factors involved in pricing.  For example, \cite{bai2019coordinating, taylor2018demand} propose a queueing model that considers earnings-sensitive independent drivers with heterogeneous reservation prices, and price-sensitive passengers with heterogeneous valuations of the service. Another important feature of ridesourcing pricing is spatial price segmentation, i.e., setting different prices in different regions to balance demand and supply in the spatial dimension \cite{WANG2019122}. \cite{zhang2020pricing} propses a sectional charging method where each active passenger shares a sectional cost  proportional to their requesting distances.}\\
In this paper, we approach the pricing-based ride-sharing (with pooling) problem through a model-free technique for ride-sharing with ride-pooling. In contrast to the model-based approaches in literature \cite{3,4,5,6}, our proposed approach can adapt to dynamic distributions of customer and driver preferences. The authors of \cite{deep_pool} provided the first model-free approach for ride-sharing with pooling, DeepPool, based on deep reinforcement learning (RL). However, DeepPool neither incorporates a dynamic demand-aware matching with a pricing strategy, nor accommodates customers’ and drivers’ conveniences. It primarily focuses on dispatching idle vehicles and adopts a greedy matching policy. To the best of our knowledge, ours is the first work that introduces a model-free approach for a distributed joint matching, pricing, and dispatching for ride-sharing where customers and drivers can weigh in their ride preferences, influencing the decision making of ride-sharing platforms.

\textcolor{blue}{
\textbf{Ridesharing Dispatch:}
Many of the studies on optimal taxi dispatching address the problem as either a variant of the vehicle routing problem (VRP) \cite{pillac2013review, hosni2014shared, jung2016dynamic} or the bipartite graph matching problem \cite{agatz2012optimization,zhan2016graph, nourinejad2016agent,tafreshian2020trip}. Under the VRP formulation, each taxi is assigned to sequentially pick up a number of passengers and under the bipartite graph formulation, each taxi is matched with the closest passenger in its vicinity.  Both modeling frameworks can easily take into account the impact of traffic conditions (in terms of travel times) on the optimal taxi dispatch plan. However, neither of the two frameworks capture the impact of taxis on normal traffic flows which can be detrimental in major cities with a high taxi mode share.  Also, neither of these approaches consider which ride requests to group together, they can potentially end up assigning requests with opposite-direction-destinations to the same vehicle.  To handle dynamic traffic conditions, \cite{alisoltani2020multi} utilize the observed average speed and update the traffic situation every 10 seconds. In \cite{vazifeh2018addressing}, authors provide a network-based solution to the following ‘minimum fleet problem’, given a collection of trips (specified by origin, destination and start time), of how to determine the minimum number of vehicles needed to serve all the trips without incurring any delay to the passengers.  However,  they do not account for any other drivers' or passengers' preferences, and thus their objective does not include major factors such as: customer's waiting time and drivers' profits. In this paper, we devise a DQN reward function that accounts for passenger-specific as well as driver-specific objectives.\\
In our approach, the integration of insertion-based matching and route planning with the distributed pricing approach allows us to avoid matching rides whose destinations are in opposite directions together. The insertion cost of a request leading to the opposite direction of a previously inserted request will be very high, and thus will come at the bottom of the list of which rides to insert into that specific route. On the other hand, if it were the only option, feeding this cost back into the driver's utility function will lead him/her to propose a very high increase in price to accomodate the extra cost of such a detour which, in turn, will cause a rejection from the passenger's side due to his/her pricing window.  The only case where the passenger may accept this ride is if they are willing to tolearet both the extra cost and time delay (according to their utility function in Section \ref{decide}), which would mean the customer will end up satisfied with the service and at the same time the driver will be compensated for the extra fuel cost incurred by the extra pay. In this manner, the matching, route planing, and pricing components work in tandem with each other to reach a common ground solution that is favorable by and profiatble to both parties.}\\
This paper utilizes the dispatch of idle vehicles using a Deep Q-Network (DQN) framework as in \cite{deep_pool}. %Depending on the DQN, we decide on the pricing by vehicles as well as the acceptance or rejection of rides by customers. 
The goal of our approach is to influence the customer and vehicle utility functions, utilizing an optimal dispatching framework, to \textcolor{blue}{(i) achieve convenient pricing and matching decisions, (ii) optimize vehicles' route planning (iii) re-position idle vehicles to areas of predicted high demand, (iv) maximize the profits for both drivers and customers and (v) reduce the customers’ waiting time, travel time, and vehicles' idle driving and overall distance. Depending on the DQN, the pricing decisions are made where drivers' can add additional price if the destination location of the passengers is in a location of a predicted low demand (i.e. future reward) as explained in Section \ref{propose}. } Further, the DQN takes into account the profits of the vehicles (as part of its objective functions) and thus is affected by both the pricing and matching decisions. Thus, the three sets of algorithms are inter-connected with each other. 
\vspace{-.1in}
\subsection{\textcolor{blue}{Contributions}}
The code for this work is available on Github\footnote{https://github.itap.purdue.edu/Clan-labs/Dynamic\_Matching\_RS}. The key contributions in this paper can be summarized as: 
\begin{itemize}[leftmargin = *]
	\item We present a novel dynamic, Demand-Aware and Pricing-based Matching and route planning (DARM) framework that is scalable up to the maximum capacity per vehicle in the initial assignmnt phase.In the optimization phase, this algorithm takes into account the near-future demand as well as the pricing associated with each ride in order to improve the route-planning by eliminating rides heading towards opposite directions and applying insertion operations to vehicles' current routes. 
	\item In addition to our matching and route-planning (DARM) framework, we integrate a novel Distributed Pricing approach for Ride-Sharing -with pooling- (DPRS) framework where, based on their convenience, customers and drivers get to weigh-in on the decision-making of a particular ride. The key idea is that the passengers are offered price based on the additional distance given the previous matched passengers thus prioritizing the passengers which will have intersections in the routes to be grouped together. %DPRS approach is built on top of a distributed model-free approach, DeepPool in \cite{deep_pool}, and utilizes its dispatching algorithm of idle vehicles using Deep Q-learning (DQN).
	\item In the DPRS framework, drivers are allowed to propose a price based on the location of the ride (source and destination) that accounts for the reward of DQN based on the destination location. Similarly, customers can either accept or reject rides based on their pricing threshold, timing preference, type of vehicle, and number of people to share a ride with. 
	\item Our joint (DARM + DPRS) framework increases the profit margins of both customers and drivers,  and the profits are also fed back to the reinforcement learning utility functions that  influence the Q-values learnt using DQN for making the vehicles' dispatch decisions. The optimization problem is formulated such that our novelty framework minimizes the rejection rate, customers' waiting time, vehicles' idle time, total number of vehicles to reduce traffic congestion,  fuel consumption,  and maximizes the vehicle's profit.
	\item  Through experiments using real-word dataset of New York City's taxi trip records \cite{10}  (15 million trips), we simulate the ride-sharing system with dynamic matching, demand-aware route planning and distributed pricing strategy. We show that our novel Joint (DARM + DPRS) framework provides up to $10$ times more profits for drivers, while maintaining minimal waiting times for customers when compared to various baselines. In addition, our framework shows a significant improvent in fleet utilization, as it uses only 50\% of the vehicles allowed by the system to fulfill up to 90\% of the demand, while keeping most of the vehicles occupied more than 80\% of the time, which brings their idle time to the minimum. We note that the three components of pricing, matching, and dispatching influence each other, and are tightly coupled. 
	%This is challenging as the overall matching  and pricing decisions as well as the acceptance rate greatly impact the ride-sharing decisions and vice versa, as they are not independent.
\end{itemize}
\vspace{-.1in}
\subsection{\textcolor{blue}{Organization}}
The rest of this paper is organized as follows: Section \ref{joint} describes the overall architecture of our framework as well as the model parameters. In Section \ref{darm}, we explain our dynamic, demand-aware, and pricing-based approach for matching and route planning. Section \ref{pricing} provides details for our pricing strategy, including the customers and drivers' utility functions and decision-making processes. In Section \ref{dqn_algo}, we decribe the DQN-based approach we utilized for dispatching vehicles. Simulation setup as well as experimental results are presented in Section \ref{results}. Finally, Section \ref{conc} concludes the paper.

==> learn.tex <==
\begin{tikzpicture}
\begin{axis}[
tick align=outside,
x grid style={white!69.0196078431373!black},
xlabel={Training step},
xmajorgrids,
xmin=-1122, xmax=23562,
xtick style={color=white!69.0196078431373!black},
y grid style={white!69.0196078431373!black},
ylabel={Average Q-Max},
ymajorgrids,
ymin=-3.07121731743086, ymax=67.3191211140041,
ytick style={black}
]
\addplot [line width=0.9pt, blue]
table {%
	0 0.149212122
	75.0501672240803 0.141698318863934
	150.100334448161 0.128343520361638
	225.150501672241 0.149890086097368
	300.200668896321 0.134391917861099
	375.250836120401 0.214585461543176
	450.301003344482 0.246142712461059
	525.351170568562 0.364775630209777
	600.401337792642 0.338609105531161
	675.451505016722 0.423610686106841
	750.501672240803 0.417411903059881
	825.551839464883 0.383865966019961
	900.602006688963 0.376678985722963
	975.652173913043 0.351314161603199
	1050.70234113712 0.157906056324347
	1125.7525083612 0.607206934899323
	1200.80267558528 0.623817616046654
	1275.85284280936 1.0435193461814
	1350.90301003344 1.15811315094528
	1425.95317725753 1.41897896470618
	1501.00334448161 1.43040616768848
	1576.05351170569 1.6203934657751
	1651.10367892977 1.7959971657968
	1726.15384615385 2.48623692139848
	1801.20401337793 2.75658734694735
	1876.25418060201 2.18768480592351
	1951.30434782609 1.76303005922851
	2026.35451505017 2.79964854148971
	2101.40468227425 2.74463791918774
	2176.45484949833 3.46700724909454
	2251.50501672241 3.2665401998325
	2326.55518394649 3.98373530551264
	2401.60535117057 4.41545649935192
	2476.65551839465 5.40862711078577
	2551.70568561873 5.33734406826906
	2626.75585284281 6.37018301963726
	2701.80602006689 6.71645357591857
	2776.85618729097 7.19090563819404
	2851.90635451505 7.67011368555634
	2926.95652173913 7.2863766721537
	3002.00668896321 7.85857933995343
	3077.05685618729 7.50342327377622
	3152.10702341137 7.34917463082379
	3227.15719063545 9.6658077820443
	3302.20735785953 10.7180788957934
	3377.25752508361 9.96558180716002
	3452.30769230769 10.0218656313818
	3527.35785953177 11.2796007468355
	3602.40802675585 11.242295597105
	3677.45819397993 11.4499346446278
	3752.50836120401 11.6521740120967
	3827.55852842809 12.9115152143432
	3902.60869565217 13.0037847644154
	3977.65886287625 12.1111467180795
	4052.70903010033 12.6966123528094
	4127.75919732441 12.8549308645733
	4202.8093645485 12.2213284831425
	4277.85953177258 12.0164625873778
	4352.90969899666 11.9053384992569
	4427.95986622074 14.3988951760724
	4503.01003344482 13.1968123093381
	4578.0602006689 15.8527322530904
	4653.11036789298 16.497979117702
	4728.16053511706 17.6460585304627
	4803.21070234114 17.3450519774215
	4878.26086956522 18.7249875452712
	4953.3110367893 18.4952491527875
	5028.36120401338 23.7794007793329
	5103.41137123746 24.3279014053644
	5178.46153846154 25.2020371046231
	5253.51170568562 24.7267080282798
	5328.5618729097 23.8355748096111
	5403.61204013378 25.6749340896354
	5478.66220735786 23.8069446952259
	5553.71237458194 25.801204525443
	5628.76254180602 27.6072024868764
	5703.8127090301 27.5098745516664
	5778.86287625418 26.3210981515601
	5853.91304347826 28.7683317058144
	5928.96321070234 28.4018256297826
	6004.01337792642 33.3203979363805
	6079.0635451505 35.1040249381541
	6154.11371237458 36.541459887228
	6229.16387959866 36.5286720038715
	6304.21404682274 36.8461803697236
	6379.26421404682 36.9770619633454
	6454.3143812709 38.0629939415163
	6529.36454849498 38.8137419574053
	6604.41471571906 36.6747181794042
	6679.46488294314 36.4327508117021
	6754.51505016722 34.4758902268162
	6829.5652173913 32.291709720376
	6904.61538461538 31.9771714603283
	6979.66555183947 33.4470935318008
	7054.71571906355 32.50414158651
	7129.76588628763 33.4071623130464
	7204.81605351171 34.1607103959842
	7279.86622073579 33.7343302600284
	7354.91638795987 37.3657791805267
	7429.96655518395 37.4202042104513
	7505.01672240803 42.3304386448628
	7580.06688963211 43.6424192506869
	7655.11705685619 45.6346521163054
	7730.16722408027 45.1889949194388
	7805.21739130435 48.8560041315361
	7880.26755852843 50.4044625952237
	7955.31772575251 53.7381498574523
	8030.36789297659 53.6425540397743
	8105.41806020067 53.6485371739496
	8180.46822742475 52.898155026896
	8255.51839464883 55.7251461193958
	8330.56856187291 55.2744847995263
	8405.61872909699 60.4409848251469
	8480.66889632107 61.2872181093616
	8555.71906354515 60.5523448236225
	8630.76923076923 57.7051105225269
	8705.81939799331 64.1195602762116
	8780.86956521739 54.8350382332782
	8855.91973244147 55.1674773655471
	8930.96989966555 57.4281358239708
	9006.02006688963 55.7585354007093
	9081.07023411371 53.2878309432758
	9156.12040133779 56.5908789216541
	9231.17056856187 53.0272946863729
	9306.22073578595 52.4886736996959
	9381.27090301003 47.5144066488326
	9456.32107023411 49.9891920081499
	9531.37123745819 50.88506338711
	9606.42140468227 50.2152227010376
	9681.47157190636 48.8509053500967
	9756.52173913044 45.9267840490577
	9831.57190635451 46.9273943986682
	9906.6220735786 46.0431212550176
	9981.67224080268 43.9979165611139
	10056.7224080268 43.7887773708991
	10131.7725752508 43.0456687891673
	10206.8227424749 49.9142704130273
	10281.872909699 42.1229872539544
	10356.9230769231 42.1171581178145
	10431.9732441472 41.0971920816883
	10507.0234113712 42.5075128270209
	10582.0735785953 42.8876944401121
	10657.1237458194 40.3447756161141
	10732.1739130435 41.3125825176378
	10807.2240802676 40.1333941005433
	10882.2742474916 41.1596177965719
	10957.3244147157 42.5847685531654
	11032.3745819398 40.602169083351
	11107.4247491639 40.5174746300149
	11182.474916388 41.4423701167747
	11257.525083612 41.8617128854803
	11332.5752508361 40.7638441029994
	11407.6254180602 40.1283502672102
	11482.6755852843 39.266565650408
	11557.7257525084 37.9875105112788
	11632.7759197324 34.327030172387
	11707.8260869565 35.5993191722247
	11782.8762541806 33.7835541722498
	11857.9264214047 36.7452099606852
	11932.9765886288 36.2272239752554
	12008.0267558528 37.1389214835163
	12083.0769230769 36.7448701235983
	12158.127090301 42.1186221163031
	12233.1772575251 43.3156341018945
	12308.2274247492 43.7856541044884
	12383.2775919732 43.164238059768
	12458.3277591973 43.0067801543099
	12533.3779264214 40.3352696013011
	12608.4280936455 43.5822461838307
	12683.4782608696 43.2983011337835
	12758.5284280936 40.7198625093214
	12833.5785953177 40.6053086132319
	12908.6287625418 39.3564100028755
	12983.6789297659 36.0878328185486
	13058.72909699 37.5630657014989
	13133.779264214 40.7613404556911
	13208.8294314381 38.7417758012735
	13283.8795986622 39.5947547800938
	13358.9297658863 37.7280812631531
	13433.9799331104 38.5049749978309
	13509.0301003344 39.2341832084923
	13584.0802675585 38.9514712448992
	13659.1304347826 36.5977652467724
	13734.1806020067 36.1570384871321
	13809.2307692308 38.1051579826948
	13884.2809364549 37.1753278273888
	13959.3311036789 39.4918731321141
	14034.381270903 38.9623930927365
	14109.4314381271 39.8191083774372
	14184.4816053512 42.8478004667429
	14259.5317725753 43.5823784188228
	14334.5819397993 42.0933161827786
	14409.6321070234 44.5940822569858
	14484.6822742475 42.7201233050777
	14559.7324414716 49.4063434536695
	14634.7826086957 45.5402934578565
	14709.8327759197 42.197917754737
	14784.8829431438 41.184896967058
	14859.9331103679 41.8062088115761
	14934.983277592 40.0220786735215
	15010.0334448161 40.5158303429083
	15085.0836120401 40.8574073851232
	15160.1337792642 42.382944381875
	15235.1839464883 40.034786288327
	15310.2341137124 43.7247618490647
	15385.2842809365 42.7029505358157
	15460.3344481605 42.0510661881899
	15535.3846153846 41.0631313036341
	15610.4347826087 43.2229963919063
	15685.4849498328 41.3441928375388
	15760.5351170569 44.5634512396049
	15835.5852842809 42.0829021575274
	15910.635451505 41.2894523537175
	15985.6856187291 39.4623036023519
	16060.7357859532 40.3244103583572
	16135.7859531773 38.5594510056957
	16210.8361204013 40.6785417472982
	16285.8862876254 39.9422792351479
	16360.9364548495 39.9567561034774
	16435.9866220736 37.2712268752813
	16511.0367892977 39.5642079467094
	16586.0869565217 36.7322526102318
	16661.1371237458 39.3918258515087
	16736.1872909699 38.6470011890952
	16811.237458194 37.4493374468404
	16886.2876254181 38.3445026840053
	16961.3377926421 38.920500571045
	17036.3879598662 40.4304174818742
	17111.4381270903 37.5811725904545
	17186.4882943144 38.4479722826439
	17261.5384615385 37.5518276894247
	17336.5886287625 39.4073456764201
	17411.6387959866 36.1918678908666
	17486.6889632107 38.6568584084307
	17561.7391304348 34.518495416321
	17636.7892976589 35.9234613010464
	17711.8394648829 35.385689940239
	17786.889632107 35.7332157140731
	17861.9397993311 39.5263218356735
	17936.9899665552 36.436610451695
	18012.0401337793 38.6654708124681
	18087.0903010033 33.9346845561553
	18162.1404682274 34.7165213454323
	18237.1906354515 34.3051334641605
	18312.2408026756 35.916033072806
	18387.2909698997 36.9363206939935
	18462.3411371237 35.957009609935
	18537.3913043478 36.633608330507
	18612.4414715719 35.6072702335313
	18687.491638796 36.2880650540336
	18762.5418060201 36.130219085256
	18837.5919732441 34.8407784123414
	18912.6421404682 38.329308089736
	18987.6923076923 37.901105799375
	19062.7424749164 38.2755123645895
	19137.7926421405 38.3399501072137
	19212.8428093645 39.0051887231308
	19287.8929765886 37.9305831125229
	19362.9431438127 38.0783635598115
	19437.9933110368 38.6241328211809
	19513.0434782609 39.1522699372316
	19588.093645485 40.4948339752588
	19663.143812709 39.6389766293742
	19738.1939799331 41.5365721918251
	19813.2441471572 39.5793345632038
	19888.2943143813 39.7476216524045
	19963.3444816054 40.3828144578829
	20038.3946488294 40.6361992898706
	20113.4448160535 37.7975011637449
	20188.4949832776 35.4719829710699
	20263.5451505017 35.3032007612119
	20338.5953177258 34.2332012034614
	20413.6454849498 34.6415869194715
	20488.6956521739 37.2829361316719
	20563.745819398 33.8429777878978
	20638.7959866221 35.8698448627566
	20713.8461538462 34.8735114313289
	20788.8963210702 36.0999561311641
	20863.9464882943 33.8996144829164
	20938.9966555184 34.7458048167857
	21014.0468227425 34.2472133190981
	21089.0969899666 36.0689417727079
	21164.1471571906 33.2785128157071
	21239.1973244147 38.4475419810626
	21314.2474916388 35.5243267877031
	21389.2976588629 36.6818494428457
	21464.347826087 36.3223524138836
	21539.397993311 37.8513842514752
	21614.4481605351 38.1076027512448
	21689.4983277592 38.3052732155286
	21764.5484949833 37.5922260846818
	21839.5986622074 34.7173163645145
	21914.6488294314 36.5117987420317
	21989.6989966555 36.6454431322173
	22064.7491638796 36.7882687189729
	22139.7993311037 36.1571596873687
	22214.8494983278 33.7607176320945
	22289.8996655518 34.0706187996483
	22364.9498327759 33.6968938548012
	22440 36.61724842
};
\end{axis}

\end{tikzpicture}
%\caption{Convergence of Q-values during training (at approximately 15k training steps.}\label{fig:Learning Curve}
%\end{figure}

==> work.tex <==
%Utilizing an operation called \textit{insertion} to solve such a highly dynamic problem has been proven, in literature, to be both effective and efficient \cite{12,14,23,30,32,35,38,40-37,44}. The \textit{insertion} operation aims to accommodate the newly arriving request by inserting its pickup (i.e., origin) and its drop-off (i.e., destination) locations into a vehicle’s route. The main issue with the state-of-the-art route planning methods \cite{10-DA,12,40-37} is that it operates in a greedy fashion to optimize its objectives, which means each insertion operation only optimizes the objective function upon the \textit{current} arranged request leading to low performance over the long run. Moreover, most of the approximation algorithms that provide solutions to the route planning problem are limited to only two requests per vehicle such as the settings in \cite{np,np2,DARP}. In \cite{DARP}, the authors improve the effectiveness of route planning for shared mobility through taking into consideration the demand in near future (e.g., future 90 minutes), thus overcoming the short sightedness problem of the insertion operator. However, the Demand-Aware Route Planning (DARP) in \cite{DARP} is still limited to only two rides per vehicle in the initial assignment phase. In addition, it does not enforce constraints on which rides can be grouped together, which may result in grouping rides whose destinations are in opposite directions; thus resulting in large detours (boosting the travel distance), as well as extra fuel and energy consumption per vehicle. Therefore, a robust framework is essential to achieve a dynamic and demand-aware matching framework that optimizes for the overall fleet's profits and its total travelling distance. Finally, the overall problem for ride-sharing requires interconnected decisions of matching, pricing, and dispatching, and is the focus of this paper. 

\textcolor{blue}{
%\textbf{Urban Transportation:}
%Some papers aim to study the practical impacts of the modeling techniques of DARPs,  for instance, \cite{GARAIX201062} discussed the problem of the graph representation of the road network where arcs are computed according to only a single criterion, for example, travel time; which could eliminate some possible routes from consideration. \\
%The majority of articles in literature consider static and deterministic Dial-A-Ride Problems (DARP)s.  The main focus of these aarticles is on algorithmic advancement where the typical setting considers a homogeneous fleet of vehicles,  passengers' pick-up and drop-off time windows,  maximum passenger ride time,  maximum route duration, and vehicle capacity.  (e.g.,  \cite{ PARRAGH20101129, PARRAGH2013490, CHASSAING2016119, ritzinger2016dynamic}).  Some papers include these requirements as hard constraints in their optimization models (e.g.,  \cite{ CHASSAING2016119,ritzinger2016dynamic}), while others may allow violations that are then penalized in the objective function so as to be avoided as much as possible \cite{urra2015hyperheuristic}.  Most of the remaining papers focus on the modeling issues regarding new problem features motivated by new applications of DARPs or real needs in practice \cite{MOLENBRUCH201758}, \cite{schonberger2017scheduling}.  Some papers aim to study the practical impacts of the modeling techniques of DARPs,  for instance, \cite{GARAIX201062} discussed the problem of the graph representation of the road network where arcs are computed according to only a single criterion, for example, travel time; which could eliminate some possible routes from consideration. \\
%In \cite{zhan2016graph},  the taxi trip data in New York City are used to quantitatively examine the gap between the current system performance and the theoretically optimal system. model-based so they can compute theoretical bound. However, this study only considers taxi servie that serve one ride at a time and does not address issues that arise with pooling or shareability.  However, in \cite{santi2014quantifying},  authors introduce the notion of shareability network, which allows modelling the collective benefits of sharing as a function of passenger inconvenience,  and  they conclde the potential of a new taxi system in which trips are routinely shareable while keeping passenger discomfort low in terms of prolonged travel time.\\
%As conclusded in \cite{HO2018395},  Dynamic and Stochastic DARPs appear to be the most challenging,  which is the focus of our paper, regarding the difficulties arising from the modeling of a combination of stochastic components,  the evaluations of outcomes under a large number of scenarios,  the integration of stochastic processes and optimization algorithms,  and the timely provision of highquality solutions for recovery.\\
%
%\textbf{RideSourcing Matching and Pricing:}
%The matching problem in urban transportation has been widely studies in literature,  \cite{agatz2012optimization} provides a review of optimization approaches in dynamic ride-sharing.  However, most of these approaches do not consider the preferences of both parties, they mostly optimize for the service provider profitability.  In our approach, matches must be time-feasible,  where both the rider’s and the driver’s travel windows are respected. The assignment problem has been studied extensively in the literature with algorithmic approaches abound, but these approaches limit their attention to what is denoted as static ride-sharing variants, where it is assumed that all driver and rider requests are known in advance prior to the execution of a matching process as in \cite{herbawi2011evolutionary, CORTES2010711}.  In \cite{alonso2017demand},  authors propose a solution for the matching problem by identifying cliques of the vehicle-pasenger graph as the potential trips. Then, they formalize optimal the assignment problem as an integer linear problem (ILP). However,  they do not address dynamic route-planning where new ride requests can be served by a vehicle that might be already assigned a trip as long as it has vacant seats. In any practical dynamic ride-share implementation, new riders and drivers continuously enter and leave the system.  Therefore,not all relevant offers and requests may be known at the time the ride-share provider executes an algorithm for planning ride-sharing arrangements. In recent years, several authors have addressed this issue in dynamic ride-sharing.
%
%Amey (2011) studies the ride-share potential at the MIT campus
%in Cambridge, Massachusetts. Given the home locations and time
%schedules of the faculty and staff, the author identifies potential
%ride-share arrangements in which two commuters share a trip together. The ride-share match optimization in this case must not
%only decide on the assignment of riders to drivers but also assign
%a role to each of the participants. It is therefore not possible to
%model this problem using bipartite matching.
%
%In \cite{AGATZ20111450}, authors deal with this planning uncertainty by using a rolling horizon solution approach where the optimization problem to be solved includes all of the offered rides (drivers) and requested rides (riders) that are known at the time of execution and that have not yet been matched.  In a similar setting, \cite{kleiner2011mechanism} apply a rolling horizon solution approach as well where arrangements are committed as late as possible given the time considerations.  This is not always applicable in real-time and can lead to customer unsatisfaction on the long run. 
%Moreover, neither drivers' nor customers' preferences are taken into consideration in the decision-making process. \\
%
%They present an auctionbased solution mechanism that takes into account the individual
%preferences of the participants for ride-share partners and rides
%
%Regarding the pricing problem, there are various ways to divide the trip costs between the ride-share partners.  \cite{geisberger2009fast} suggests to divide the cost of the shared part of the trip evenly between the ride-share partners.  In \cite{AGATZ20111450},  authors propose a way to allocate the costs of the joint trip that is proportional to the distances of the separate trips.  \cite{kleiner2011mechanism} proposes an auction-based mechanism to determine the driver’s compensation. This approach takes into account the different ride valuations of individual riders.  Most works in literature study ride-sourcing pricing based on the steady-state equilibrium approach.  In \cite{cachon2017role}, authors study surge-pricing as a revenue management strategy. They consider a two-period newsvendor model to study the impact of contractual agreements for ‘self-scheduling’ agents, i.e., drivers that choose their own work-shifts in ride-sourcing markets.  However,  the requirements for a stationary equilibrium as well as the assumption of time-invariant fleet size are strict and rarely prevailing in reality. \\
%The authors in \cite{nourinejad2019ride} consider a non-equilibrium two-sided markets, however they propose a model-based approach that introduces a three-state model (riders, vacant ride-sourcing vehicles, and occupied ride-sourcing vehicles) where the arrivals of vehicles and riders are endogenously dependent on the market state. Many researchers focus on the interactions and endogeneity between various factors involved in pricing.  For example, \cite{bai2019coordinating, taylor2018demand} propose a queueing model that considers earnings-sensitive independent drivers with heterogeneous reservation prices, and price-sensitive passengers with heterogeneous valuations of the service.
%e. Taylor (2018) also
%uses a queueing formulation with a two-point distribution for passenger and driver valuation, derives the demand rate and
%number of drivers in equilibrium for a given price and wage, and finds that uncertainty in passenger delay sensitivity and
%driver independence may change the intuitive price and wage prescriptions. 
%Another important feature of ridesourcing pricing is spatial price segmentation, i.e., setting different prices in different regions to balance demand and supply in the spatial dimension \cite{WANG2019122}.\\
%\textbf{Ridesharing Dispatch:}
%%network-saxi dispatch model that takes into account the interrelated impact of normal traffic flows and taxi dynamics while optimizing for an effective disatch system: Model based and no pooling
%%
%Many of the studies on optimal taxi dispatching address the problem as either a variant of the vehicle routing problem (VRP) \cite{pillac2013review, hosni2014shared, jung2016dynamic} or the bipartite graph matching problem \cite{agatz2012optimization,zhan2016graph, nourinejad2016agent}. Under the VRP formulation, each taxi is assigned to sequentially pick up a number of passengers and under the bipartite graph formulation, each taxi is matched with the closest passenger in its vicinity.  Both modeling frameworks can easily take into account the impact of traffic conditions (in terms of travel times) on the optimal taxi dispatch plan. However, neither of the two frameworks capture the impact of taxis on normal traffic flows which can be detrimental in major cities with a high taxi mode share.  In \cite{vazifeh2018addressing}, authors provide a network-based solution to the following ‘minimum fleet problem’, given a collection of trips (specified by origin, destination and start time), of how to determine the minimum number of vehicles needed to serve all the trips without incurring any delay to the passengers.  However,  they do not account for any other driver or passenger preferences.
}
